Periodic fluctuations in deep water formation due to sea ice

During the last ice age several quasi-periodic abrupt warming events took place. Known as Dansgaard-Oeschger (DO) events their effects were felt globally, although the North Atlantic experienced the largest temperature anomalies. Paleoclimate data shows that the fluctuations often occurred right after massive glacial meltwater releases in the North Atlantic and in bursts of three or four with progressively decreasing strengths. In this study a simple dynamical model of an overturning circulation and sea ice is developed with the goal of understanding the fundamental mechanisms that could have caused the DO events. Interaction between sea ice and the overturning circulation in the model produces self-sustained oscillations. Analysis and numerical experiments reveal that the insulating effect of sea ice causes the ocean to periodically vent out accumulated heat in the deep ocean into the atmosphere. Subjecting the model to idealized freshwater forcing mimicking Heinrich events causes modulation of the natural periodicity and produces burst patterns very similar to what is observed in temperature proxy data. Numerical experiments with the model also suggests that the characteristic period of 1,500 years is due to the geometry, or the effective heat capacity, of the ocean that comes under sea ice cover.

==> bibitems.tex <==
\begin{thebibliography}{10}

\bibitem{aagard_1985}
K.~Aagaard, J.~H. Swift, and E.~C. Carmack.
\newblock Thermohaline circulation in the {A}rctic {M}editerranean seas.
\newblock {\em Journal of Geophysical Research}, 90(C3):4833--4846, 1985.

\bibitem{adkins2002}
J.~F. Adkins, K.~McIntyre, and D.~P. Schrag.
\newblock The salinity, temperature, and {\oxy} of the glacial deep ocean.
\newblock {\em Science}, 298:1769--73, 2002.

\bibitem{alley_2007}
R.~B. Alley.
\newblock Wally was right: Predictive ability of the north atlantic "conveyor
  belt" hypothesis for abrupt climate change.
\newblock {\em Annu. Rev. Earth Planet. Sci.}, 35:241--272, 2007.

\bibitem{alley_2001}
R.~B. Alley, S.~Anandakrishnan, and P.~Jung.
\newblock Stochastic resonance in the {N}orth {A}tlantic.
\newblock {\em Paleooceanography}, 16:190--198, 2001.

\bibitem{alley_1994}
R.~B. {Alley} and D.~R. {MacAyeal}.
\newblock Ice-rafted debris associated with binge/purge oscillations of the
  {L}aurentide {I}ce {S}heet.
\newblock {\em Paleooceanography}, 9(4):503--511, 1994.

\bibitem{berger1991}
A.~Berger and M.~F. Loutre.
\newblock Insolation values for the climate of the last 10 million years.
\newblock {\em Quaternary Science Reviews}, 10:297--317, 1991.

\bibitem{bond2001}
G.~Bond, B.~Kromer, J.~Beer, R.~Muscheler, M.~N. Evans, W.~Showers, S.~Hoffman,
  R.~Lotti, I.~Hajdas, and G.~Bonani.
\newblock Persistent solar influence on {N}orth {A}tlantic climate during the
  {H}olocene.
\newblock {\em Science}, 294:2130, 2136 2001.

\bibitem{bond_lotti_1995}
G.~Bond and R.~Lotti.
\newblock Iceberg discharges into the {N}orth {A}tlantic on millennial time
  scales during the last glaciation.
\newblock {\em Science}, 267:1005--1010, 1995.

\bibitem{bond1997}
G.~Bond, W.~Showers, M.~Cheseby, R.~Lotti, P.~Almasi, P.~deMenocal, P.~Priore,
  H.~Cullen, I.~Hajdas, and G.~Bonani.
\newblock A pervasive millennial-scale cycle in north atlantic holocene and
  glacial climates.
\newblock {\em Science}, 278:1257, 1266 1997.

\bibitem{bond1999}
G.~Bond, W.~Showers, M.~Elliot, M.~Evans, R.~Lotti, I.~Hajdas, G.~Bonani, and
  S.~J. Johnsen.
\newblock The {N}orth {A}tlantic's 1-2kyr climate rhythm: relation to heinrich
  events, dansgaard/oeschger cycles and the {L}ittle {I}ce {A}ge.
\newblock {\em Geophysical Monograph}, 112:35--57, 1999.

\bibitem{braun2005}
H.~Braun, M.~Christl, S.~Rahmstorf, A.~Ganopolski, A.~Mangini, C.~Kubatzki,
  K.~Roth, and B.~Kromer.
\newblock Possible solar origin of the 1,470-year glacial climate cycle
  demonstrated in a coupled model.
\newblock {\em Nature}, 438:208--211, 2005.

\bibitem{broecker1992}
W.~Broecker.
\newblock Upset for {M}ilankovitch theory.
\newblock {\em Nature}, 359:779--780, 1992.

\bibitem{broecker2006}
W.~Broecker.
\newblock Was the {Y}ounger-{D}ryas triggered by a flood?
\newblock {\em Science}, 312(5777):1146--1148, 2006.

\bibitem{broecker1985}
W.~Broecker, D.~M. Peteet, and D.~Rind.
\newblock Does the ocean-atmosphere system have more than one stable mode of
  operation?
\newblock {\em Nature}, 315:21--26, 1985.

\bibitem{budyko_1969}
M.~Budyko.
\newblock The effect of solar radiation variations on the climate of the earth.
\newblock {\em Tellus}, XXI:611--619, 1969.

\bibitem{claussen_etal_2003}
M.~Claussen, A.~Ganopolski, and V.~Brovkin.
\newblock Simulated global-scale response of the climate system to
  {D}ansgaard/{O}eschger and {H}einrich events.
\newblock {\em Climate Dynamics}, 21:361--370, 2003.

\bibitem{claussen_2002}
M.~Claussen, L.~A. Mysack, A.~J. Weaver, M.~Crucifix, T.~Fichefet, M.~F.
  Loutre, S.~L. Weber, J.~Alcamo, V.~A. Alexeev, A.~Berger, R.~Calov,
  A.~Ganopolski, H.~Goose, G.~Lohmann, F.~Lunkeit, I.~I. Mokhov, V.~Petoukhov,
  P.~Stone, and Z.~Wang.
\newblock Earth system models of intermediate complexity: closing the gap in
  the spectrum of climate system models.
\newblock {\em Climate Dynamics}, 18:579--586, 2002.

\bibitem{clemens1997}
S.~C. Clemens and R.~Tiedemann.
\newblock Eccentricity forcing of pliocene-early pleistocene climate revealed
  in a marine oxygen-isotope record.
\newblock {\em Nature}, 385(801-804), 1997.

\bibitem{crowley.etal.1994}
T.~Crowley and K-Y Kim.
\newblock Milankovitch forcing of the last interglacial sea level.
\newblock {\em Science}, 265(5178):1566--1568, 1994.

\bibitem{dansgaard1993}
W.~Dansgaard.
\newblock Evidence for general instability of past climate from a 250-kyr
  ice-core record.
\newblock {\em Nature}, 364:218--220, 1993.

\bibitem{verdiere2006}
C.~de~Verdi\`{e}re, M.~B. Jelloul, and F.~Sevellec.
\newblock Bifurcation structure of thermohaline millennial oscillations.
\newblock {\em Journal of Climate}, 19:5777--5795, 2006.

\bibitem{dijkstra_2001}
H.~Dijkstra.
\newblock {\em Nonlinear Physical Oceanography: A Dynamical Systems Approach to
  the Large Scale Ocean Circulation and El Ni{\~n}o}.
\newblock Springer, 2001.

\bibitem{ditlevsen2009}
P.~Ditlevsen.
\newblock Bifurcation structure and noise-assisted transitions in the
  pleistocene glacial cycles.
\newblock {\em Paleooceanography}, 24, 2009.

\bibitem{fairbanks1989}
R.~G. Fairbanks.
\newblock A 17,000-year glacio-eustatic sea level record: influence of glacial
  melting rates on the younger dryas event and deep-ocean circulation.
\newblock {\em Nature}, 342(637 - 642), 1989.

\bibitem{friedrich2010}
T.~Friedrich, A.~Timmermann, L.~Menviel, O.~E. Timm, A.~Mouchet, and D.~M.
  Roche.
\newblock The mechanism behind internally generated centennial-to-millennial
  scals climate variability in an earth system model of intermediate
  complexity.
\newblock {\em Geoscientific Model Development}, 3:377--389, 2010.

\bibitem{gallup1994}
C.~D. Gallup.
\newblock The timing of high sea levels over the past 200,000 years.
\newblock {\em Science}, 263(5148):796--800, 1994.

\bibitem{gallup1999}
C.~D. Gallup.
\newblock {Sea Level Record for the Last 200,000 Years from Concordant U-Th and
  U-Pa Dates of Fossil Corals: Implications for Deep-Sea Temperature Changes
  and for Early Sea Level Rise During Termination II}.
\newblock {\em EOS Transactions}, 80(F581), 1999.

\bibitem{ganopolski_rahmstorf_2001}
A.~Ganopolski and S.~Rahmstorf.
\newblock Rapid changes of glacial climate simulated in a coupled climate
  model.
\newblock {\em Nature}, 409:153--159, 2001.

\bibitem{GT2001b}
H.~Gildor and E.~Tziperman.
\newblock A sea ice climate switch mechanism for the 100-kyr glacial cycles.
\newblock {\em Journal of Geophysical Research}, 106(C5):9117, 9133 2001.

\bibitem{gildor_2003}
H.~Gildor and E.~Tziperman.
\newblock Sea-ice switches and abrupt climate changte.
\newblock {\em Phil. Trans. R. Soc. A}, 361:1935--1944, 2003.

\bibitem{goosse1999}
H.~Goosse and T.~Fichefet.
\newblock Importance of ice-ocean interactions for the global ocean
  circulation: a model study.
\newblock {\em Journal of Geophysical Research}, 104(C10):23337--23355, 1999.

\bibitem{haarsma_2001}
R.~J. Haarsma, J.~D. Opsteegh, F.~M. Selten, and X.~Wang.
\newblock Rapid transitions and ultra-low frequency behavior in a 40 kyr
  integration with a coupled climate model of intermediate complexity.
\newblock {\em Climate Dynamics}, 17:559--570, 2001.

\bibitem{hartmann_1994}
D.~L. Hartmann.
\newblock {\em Global physical climatology}.
\newblock Academic Press, 1994.

\bibitem{hays.etal.1976}
J.~D. Hays, Imbrie~J. A., and Shackleton~N. J.
\newblock Variations in the earth's orbit: Pacemaker of the ice ages.
\newblock {\em Science}, 194(4270):1121--1132, 1976.

\bibitem{heinrich1988}
H.~Heinrich.
\newblock Origin and consequences of cyclic ice rafting in the northeast
  atlantic ocean during the past 130,000 years.
\newblock {\em Quartery Research}, 29:142--152, 1988.

\bibitem{hofmann_rahmstorf_2009}
M.~Hofmann and S.~Rahmstorf.
\newblock On the stability of the atlantic meridional overturning circulation.
\newblock {\em PNAS}, 10(1073), 2009.

\bibitem{hogg_2008}
A.~Hogg.
\newblock Glacial cycles and carbon dioxide: A conceptual model.
\newblock {\em Geophysical Research Letters}, 35, 2008.

\bibitem{hsiung1985}
J.~Hsiung.
\newblock Estimates of global oceanic meridional heat transport.
\newblock {\em J. Phys. Oceanography}, 15:1405--1413, 1985.

\bibitem{huybers2006}
P.~Huybers.
\newblock Early pleistocene glacial cycles and the integrated summer insolation
  forcing.
\newblock {\em Science}, 313:508--511, 2006.

\bibitem{huybers}
P.~Huybers and C.~Wunsch.
\newblock Obliquity pacing of the late pleistocene glacial terminations.
\newblock {\em Nature}, 434:491--494, 2005.

\bibitem{imbrie1993}
J.~Imbrie, A.~Berger, E.~A. Boyle, S.~C. Clemens, A.~Duffy, W.~R. Howard,
  G.~Kukla, J.~Kutzbach, D.~G. Martinson, A.~McIntyre, A.~C. Mix, B.~Molfino,
  J.~J. Morley, L.~C. Peterson, N.~G. Pisias, W.~L. Prell, M.~E. Raymo, N.~J.
  Shackleton, and J.~R. Toggeriler.
\newblock On the structure and origin of major glaciation cycles 2. the
  100,000-year cycle.
\newblock {\em Paleooceanography}, 8(699-735), 1993.

\bibitem{johnsen2001}
S.~J. Johnsen.
\newblock {Oxygen isotope and palaeotemperature records from six Greenland
  ice-core stations: Camp Century, Dye-3, GRIP, GISP2, Renland and NorthGRIP}.
\newblock {\em Journal of Quarternary Science}, 16(4):299, 2001.

\bibitem{jongma2007}
J.~I. Jongma, M.~Prange, H.~Ressen, and M.~Schulz.
\newblock Amplification of holocene multicentennial climate forcing by mode
  transitions in north atlantic overturning circulation.
\newblock {\em Geophysical Research Letters}, 34, 2007.

\bibitem{kageyama_2009}
M.~Kageyama, J.~Mignot, D.~Swingedouw, C.~Marzin, R.~Alkama, and O.~Marti.
\newblock Glacial climate sensitivity to different states of the atlantic
  meridional overturning circulation: Results from the {IPSL} model.
\newblock {\em Climate of the Past}, 5:551--570, 2009.

\bibitem{keeling2000}
C.~D. Keeling and T.~P. Whorf.
\newblock The 1,800-year oceanic tidal cycle: A possible cause of rapid climate
  change.
\newblock {\em Proceedings of the Natural Academy of Sciences (PNAS)},
  97:3814--3819, April 2000.

\bibitem{keith1995}
D.W. Keith.
\newblock Meridional energy transport: Uncertainty in zonal means.
\newblock {\em Tellus}, 47A:30--44, 1995.

\bibitem{kim.et.al1998}
S.~J. Kim, T.~Crowley, and A.~St{\"o}ssel.
\newblock Local orbital forcing of {A}ntarctic climate change during the last
  interglaciallocal orbital forcing of antarctic climate change.
\newblock {\em Science}, 280(5364):728--730, 1998.

\bibitem{knorr.lohmann.2003}
G.~Knorr and G.~Lohmann.
\newblock Southern {O}cean origin for the resumption of {A}tlantic thermohaline
  circulation during deglaciation.
\newblock {\em Nature}, 424:532--536, 2003.

\bibitem{laskar.et.al.2004}
J.~Laskar, P.~Robutel, F.~Joutel, M.~Gastineau, A.~C.~M. Correia, and
  B.~Levrard.
\newblock A long-term numerical solution for the insolation quantities of the
  earth.
\newblock {\em Astronomy and Astrophyiscs}, 428:261--285, 2004.

\bibitem{lean1998}
J.~Lean and D.~Rind.
\newblock Climate forcing by changing solar radiation.
\newblock {\em Journal of Climate}, 11:3069--3094, 1998.

\bibitem{lenderink1994}
G.~Lenderink and R.~J. Haarsma.
\newblock Variability and miltiple equilibria of the thermohaline circulation
  associated with deep-water formation.
\newblock {\em Journal of Physical Oceanography}, 24:1480--1493, 1994.

\bibitem{lisiecki2010}
L.~Lisiecki.
\newblock Links between eccentricity forcing and the 100,000-year glacial
  cycle.
\newblock {\em Nature Geoscience}, 3:349--352, 2010.

\bibitem{lisiecki2005}
L.~Lisiecki and M.~E. Raymo.
\newblock A pliocene-pleistocene stack of 57 globally distributed benthic d 18o
  records.
\newblock {\em Paleooceanography}, 20, 2005.

\bibitem{liu1998}
H.~S. Liu.
\newblock Phase modulation effect of the rubincam insolation variations on
  climate change.
\newblock {\em Theoretical and Applied Climatology}, 61:217--229, 1998.

\bibitem{maslin2001}
M.~Maslin, D.~Seidov, and J.~Lowe.
\newblock Synthesis of the nature and causes of rapid climate transitions
  during the quaternary.
\newblock {\em Geophysical Monograph}, 126:9--52, 2001.

\bibitem{muller1997}
R.~A. Muller and G.~MacDonald.
\newblock Spectrum of 100-kyr glacial cycle: Orbital inclination, not
  eccentricity.
\newblock {\em Proceedings of the Natural Academy of Sciences (PNAS)},
  94:8329--8334, 1997.

\bibitem{muscheler_2006}
R.~Muscheler and J.~Beer.
\newblock Solar forced {D}ansgaard/{O}eschger events?
\newblock {\em Geophysical Research Letters}, 33(L20706), 2006.

\bibitem{ngrip}
{North Greenland Ice Core Project members}.
\newblock High-resolution record of northern hemisphere climate extending into
  the last interglacial period.
\newblock {\em Nature}, 431:147--151, 2004.

\bibitem{okazaki2010}
Y.~Okazaki, A.~Timmermann, L.~Menviel, N.~Harada, A.~Abe-Ouchi, M.~O.
  Chikamoto, A.~Mouchet, and H.~Asahi.
\newblock Deepwater formation in the {N}orth {P}acific during the last glacial
  termination.
\newblock {\em Science}, 329:200--204, 2010.

\bibitem{Opsteegh1998}
J.~D. Opsteegh, R.~J. Haarsma, F.~M. Selten, and A.~Kattenberg.
\newblock A dynamic alternative to mixed boundary conditions in ocean models.
\newblock {\em Tellus}, 50A:348--367, 1998.

\bibitem{paillard1997}
D.~Paillard.
\newblock The timing of pleistocene glaciations from a simple multiple-state
  climate model.
\newblock {\em Nature}, 391:378--381, 1997.

\bibitem{paul_2002}
A.~Paul and M.~Schulz.
\newblock {\em Holocene Climate variability on centennial-to-millennial time
  scales: 2. Internal and forced oscillations as possible causes}.
\newblock Springer, 2002.

\bibitem{peterson_2000}
L.~C. Peterson, G.~H. Haug, K.~A. Hughen, and U.~R{\"o}hl.
\newblock Rapid changes in the hydrological cycle of the tropical atlantic
  during the last glacial.
\newblock {\em Science}, 290:1947--1951, 2000.

\bibitem{petit1999}
J.~R. Petit, J.~Jouzel, D.~Raynaud, N.~I. Barkov, J.~M. Barnola, I.~Basile,
  M.~Bender, J.~Chappellaz, M.~Davis, G.~Delaygue, M.~Delmotte, V.~M.
  Kotlyakov, M.~Legrand, V.~Y. Lipenkov, C.~Lorius, L.~Pepin, C.~Ritz,
  E.~Saltzman, and M.~Stievenard.
\newblock Climate and atmospheric history of the past 420,000 years from the
  {V}ostok ice core, {A}ntarctica.
\newblock {\em Nature}, 399:426--436, 1999.

\bibitem{pierce_1995}
D.~W. Pierce, T.P. Barnett, and U.~Mikolajewicz.
\newblock Competing roles of heat and freshwater flux in forcing thermohaline
  oscillations.
\newblock {\em Journal of Physical Oceanography}, 25:2046--2064, 1995.

\bibitem{rahmstorf1994}
S.~Rahmstorf.
\newblock Multiple convection patterns and thermohaline flow in an idealized
  {OGCM}.
\newblock {\em Journal of Climate}, 8:3028--3039, 1994.

\bibitem{rahmstorf_2002}
S.~Rahmstorf.
\newblock Ocean circulation and climate during the past 120,000 years.
\newblock {\em Nature}, 419:207--214, 2002.

\bibitem{rahmstorf_2003}
S.~Rahmstorf.
\newblock Timing of abrupt climate change: A precise clock.
\newblock {\em Geophysical Research Letters}, 30(10):17--2:17--4, 2003.

\bibitem{rahmstorf2005}
S.~Rahmstorf, M.~Crucifix, A.~Ganopolski, H.~Goosse, I.~Kamenkovich, R.~Knutti,
  G.~Lohmann, R.~Marsh, L.~A. Mysack, Z.~Wang, and A.~J. Weaver.
\newblock Thermohaline circulation hysteresis: A model intercomparison.
\newblock {\em Geophysical Research Letters}, 32, 2005.

\bibitem{ray2001}
N.~Ray and J.~M. Adams.
\newblock Gis-based vegetation map of the world at the last glacial maximum
  (25,000-15,000 bp)-(23rd millennium to 13th millennium bc.
\newblock {\em Internet Archaeology}, 11, 2001.

\bibitem{raymo1997}
M.~E. Raymo.
\newblock The timing of major terminations.
\newblock {\em Paleooceanography}, 12:577--585, 1997.

\bibitem{rial1999}
J.~A. Rial.
\newblock Pacemaking the ice ages by frequency modulation of the earth's
  orbital eccentricity.
\newblock {\em Science}, 285:564--568, 1999.

\bibitem{rial_saha_2008}
J.~A. Rial and R.~Saha.
\newblock Stochastic resonance, frequency modulation and the mechanisms of
  abrupt climate change in the arctic.
\newblock {\em First International Symposium on Arctic Research, Drastic Change
  Under Global Warming (ext. abs.)}, 1:94--97, 2008.

\bibitem{rial_yang_2007}
J.~A. Rial and M.~Yang.
\newblock Is abrupt climate change paced by the orbital insolation?
\newblock {\em Geophysical Monograph}, 173:167--174, 2007.

\bibitem{rooth_1982}
C.~Rooth.
\newblock Hydrology and ocean circulation.
\newblock {\em Prog. Oceanography}, 11:131--149, 1982.

\bibitem{ruddick_1996}
B.~Ruddick and L.~Zhang.
\newblock Qualitative behavior and nonoscillation of stommel's thermohaline box
  model.
\newblock {\em Journal of Climate}, 9:2768--2777, 1996.

\bibitem{ruddiman_mcintyre_1981}
W.~F. Ruddiman and A.~McIntyre.
\newblock The mode and mechanism of the last deglaciation: Oceanic evidence.
\newblock {\em Quartery Research}, 16:125--134, 1981.

\bibitem{sakai_peltier_1995}
K.~Sakai and W.~R. Peltier.
\newblock A simple model of the atlantic thermohaline circulation: Internal and
  forced variability with paleoclimatological implication.
\newblock {\em Journal of Geophysical Research}, 100:13,455--13,479, 1995.

\bibitem{sakai_peltier_1999}
K.~Sakai and W.~R. Peltier.
\newblock A dynamical systems model of the dansgaard--oeschger oscillation and
  the origin of the bond cycle.
\newblock {\em Journal of Climate}, 12:2238--2255, 1999.

\bibitem{sarnthein_2003}
M.~Sarnthein, U.~Pflaumann, and M.~Weinelt.
\newblock Past extent of sea ice in the northern {N}orth {A}tlantic inferred
  from foraminiferal paleotemperature estimates.
\newblock {\em Paleooceanography}, 18(2):1047, 2003.

\bibitem{schulz_1998}
H.~Schulz, U.~{von Rad}, and H.~Erlenkeuser.
\newblock Correlation between arabian sea and greenland climate oscillations of
  the past 110,000 years.
\newblock {\em Nature}, 393:54--58, 1998.

\bibitem{schulz2006}
M.~Schulz, M.~Prange, and A.~Klocker.
\newblock Low-frequency oscillations of the atlantic ocean meridional
  overturning circulation in a coupled climate model.
\newblock {\em Climate of the Past Discussions}, 2:801--830, 2006.

\bibitem{sellers_1969}
W.~Sellers.
\newblock A climate model based on the energy balance of the earth-atmosphere
  system.
\newblock {\em Journal of Applied Metereology}, 8:392--400, 1969.

\bibitem{severinghaus_1999}
J.~Severinghaus and E.~J. Brook.
\newblock Abrupt climate change at the end of the last glacial period inferred
  from trapper air in polar ice.
\newblock {\em Science}, 286:930--934, 1999.

\bibitem{shaffer_etal_2004}
G.~Shaffer, S.~M. Olsen, and C.~J. Bjerrum.
\newblock Ocean subsurface warming as a mechanism for coupling
  dansgaard-oeschger climate cycles and ice-rafting events.
\newblock {\em Geophysical Research Letters}, 31, 2004.

\bibitem{stocker2003}
T.~Stocker and S.~J. Johnsen.
\newblock A minimum thermodynamic model for the bipolar seesaw.
\newblock {\em Paleooceanography}, 18(4), 2003.

\bibitem{stommel}
H.~Stommel.
\newblock Thermohaline convection with two stable regimes of flow.
\newblock {\em Tellus}, 1961.

\bibitem{esat1999}
et~al. T.~M.~Esat.
\newblock Rapid fluctuations in sea level recorded at {H}uon {P}eninsula during
  the penultimate deglaciation.
\newblock {\em Science}, 283(5399):197--201, 1999.

\bibitem{thual_mcwilliams_1992}
O.~Thual and J.~McWilliams.
\newblock The catastrophe structure of thermohaline convection in a
  two-dimensional fluid model and a comparison with low-order box models.
\newblock {\em Geophysical \& Astrophysical Fluid Dynamics}, 64:67--95, 1992.

\bibitem{timmermann_2001}
A.~Timmermann, H.~Gildor, M.~Schulz, and E.~Tziperman.
\newblock Coherent resonant millennial-scale climate oscillations triggered by
  massive meltwater pulses.
\newblock {\em Journal of Climate}, 16:2569--2585, 2003.

\bibitem{wang2001}
Y.~J. Wang, H.~Cheng, R.~L. Edwards, Z.~S. An, J.~Y. Wu, C.-C Shen, and J.~A.
  Dorale.
\newblock A high-resolution absolute-dated late pleistocene monsoon record from
  {H}ulu cave, {C}hina.
\newblock {\em Science}, 294:2345--2348, 2001.

\bibitem{wang_mysak_2006}
Z.~Wang and L.~Mysak.
\newblock Glacial abrupt climate changes and dansgaard-oeschger oscillations in
  a coupled climate model.
\newblock {\em Paleooceanography}, 21(PA2001), 2006.

\bibitem{watson_lovelock_1983}
A.~Watson and J.~Lovelock.
\newblock Biological homeostasis of the global environment: the parable of
  daisyworld.
\newblock {\em Tellus}, 35B:284, 289 1983.

\bibitem{welander_1982}
P.~Welander.
\newblock A simple heat-salt oscillator.
\newblock {\em Dynamics of Atmosphere and Oceans}, 6(233-242), 1982.

\bibitem{winograd1992}
I.J. Winograd.
\newblock Continuous 500,000-year climate record from vein calcite in devils
  hole, nevada.
\newblock {\em Science}, 258(5080):255--260, 1992.

\bibitem{winton_1993}
M.~Winton and E.~S. Sarachik.
\newblock Thermohaline oscillations induced by strong steady stalinity forcing
  of ocean general circulation models.
\newblock {\em Journal of Physical Oceanography}, 23(7):1389--1410, 1993.

\bibitem{zhang_2002}
R.~Zhang.
\newblock Mechanisms of thermohaline mode switching with application to warm
  equable climates.
\newblock {\em Journal of Climate}, 15:2056--2072, 2002.

\end{thebibliography}

